On the Order Type of Scattered Context-Free Orderings

We show that if a context-free grammar generates a language whose lexicographic ordering is well-ordered of type less than $\omega^2$, then its order type is effectively computable.

==> eptcsdata.tex <==
\providecommand{\firstpage}{169}
\providecommand{\publicationstatus}{J. Leroux and J.-F. Raskin (Eds.): Tenth International Symposium\\ on Games, Automata, Logics, and Formal Verification (GandALF'19).\\
EPTCS 305, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.305.12}{10.4204/EPTCS.305.12}}

